TokenMixup: Efficient Attention-guided Token-level Data Augmentation for Transformers

Mixup is a commonly adopted data augmentation technique for image classification. Recent advances in mixup methods primarily focus on mixing based on saliency. However, many saliency detectors require intense computation and are especially burdensome for parameter-heavy transformer models. To this end, we propose TokenMixup, an efficient attention-guided token-level data augmentation method that aims to maximize the saliency of a mixed set of tokens. TokenMixup provides x15 faster saliency-aware data augmentation compared to gradient-based methods. Moreover, we introduce a variant of TokenMixup which mixes tokens within a single instance, thereby enabling multi-scale feature augmentation. Experiments show that our methods significantly improve the baseline models' performance on CIFAR and ImageNet-1K, while being more efficient than previous methods. We also reach state-of-the-art performance on CIFAR-100 among from-scratch transformer models. Code is available at https://github.com/mlvlab/TokenMixup.

==> 04_Experiments/imagenet.tex <==
\subsection{ImageNet-1K}
Performance on ImageNet-1K is evaluated on the vanilla ViT~\cite{dosovitskiy2020image} model.
The officially reported Top-1 accuracy is 81.2\%, which is achieved by using the weights pre-trained on ImageNet-21K and fine-tuned on ImageNet-1K.
By fine-tuning the model further by employing our augmentation methods, we achieve Top-1 accuracy of 82.3\% with Horizontal TokenMixup, and 82.2\% with Vertical TokenMixup.
Also note that HTM marginally increases parameter size by 0.7M, while VTM does not require any additional parameters.

==> Algorithms/htm.tex <==

\begin{algorithm}[ht!]
\caption{Horizontal TokenMixup}
\label{alg:htm}
\begin{algorithmic}[1]
    \State \textbf{Input}  : $X \in \rm I\!R^{b \times n \times d}$, $Y \in \rm I\!R^{b \times c}$, mixup / saliency threshold $\tau$ / $\rho$
    \State \textbf{Output} : $X \in \rm I\!R^{b \times n \times d}$, $Y \in \rm I\!R^{b \times c}$, ScoreNet predictions
    \State $A \gets \textrm{propagate subsequent } \ell \textrm{ layers with stop-gradient and apply attention rollout}$
    % \State $A \gets \textrm{forward self attention with stop-gradient to retrieve attention map}$
    \State $S_t \gets \frac{1}{n}\sum_{i=1}^n  A_{t,i} \:\:\:\:\:\: \textrm{s.t.} \:\: t=1,2,\ldots,n$
    \State $\hat{Y} \gets \textrm{ScoreNet}(X)$
    \State $P \gets \sum_{i=1}^c \hat{Y}_i \odot Y_i$
    \State $\tilde{X}, \tilde{Y}, \tilde{S}_t \gets$ random permutation of $X, Y, S_t$
    \For{each sample index $m = 1, 2, \ldots, b$}
    \If{$P^{(m)} < \tau$}
    \State do not perform mixup
    \Else
    \State $k \gets \sum_{t=1}^n \mathbb{1}_{\{S_t^{(m)} < \:\rho\}}$
    \State $\mathcal{U} \gets $ bottom $k$ token indices of $X^{(m)}$ \:\: w.r.t \:\:$S_t^{(m)}$
    \State $\mathcal{V} \gets $ top $k$ token indices of $\tilde{X}^{(m)}$ \:\:w.r.t\:\: $\tilde{S}_t^{(m)}$
    \State $X^{(m)}_{t \in \mathcal{U}} \gets \tilde{X}^{(m)}_{t \in \mathcal{V}} $  
    \State $Y^{(m)} \gets\frac{\sum_{t=1}^n \mathbb{1}_{\{t \notin \mathcal{U}\}} \cdot S_t^{(m)}}{\sum_{t=1}^n \mathbb{1}_{\{t \notin \mathcal{U}\}} \cdot S_t^{(m)} + \mathbb{1}_{\{t \in \mathcal{V}\}} \cdot \tilde{S}_t^{(m)}}\cdot Y^{(m)} + \frac{\sum_{t=1}^n \mathbb{1}_{\{t \in \mathcal{V}\}} \cdot \tilde{S}_t^{(m)}}{\sum_{t=1}^n \mathbb{1}_{\{t \notin \mathcal{U}\}} \cdot S_t^{(m)} + \mathbb{1}_{\{t \in \mathcal{V}\}} \cdot \tilde{S}_t^{(m)}}\cdot \tilde{Y}^{(m)}$
    \EndIf
    \EndFor
    
    \State \textbf{return} $X$, $Y$, $\hat{Y}$
\end{algorithmic}
\end{algorithm}




% \begin{algorithm}[h]
% \caption{TokenMixer - unrolled algorithm}
% \label{alg:token_mixup}
% \begin{algorithmic}[1]
%     \State \textbf{Input}  : $X \in \rm I\!R^{b \times n \times d}$, $Y \in \rm I\!R^{b \times c}$, mixup / saliency threshold $\tau$ / $\rho$, softness $\lambda$
%     \State \textbf{Output} : $X \in \rm I\!R^{b \times n \times d}$, $Y \in \rm I\!R^{b \times c}$, ScoreNet Loss 
%     \State $A \gets \textrm{propagate subsequent } l \textrm{ layers with stop-gradient and apply attention rollout}$
%     % \State $A \gets \textrm{forward self attention with stop-gradient to retrieve attention map}$
%     \State $S_t \gets \frac{1}{n}\sum_{i=1}^n  A_{t,i} \:\:\:\:\:\: \textrm{s.t.} \:\: t=1,2,\ldots,n$
%     \State $\hat{Y} \gets \textrm{ScoreNet}(X)$
%     \State $P \gets \sum_{i=1}^c \hat{Y}_i \odot Y_i$
%     \State $\tilde{X}, \tilde{Y}, \tilde{S}_t \gets$ random permutation of $X, Y, S_t$
%     \For{each sample index $m = 1, 2, \ldots, b$}
%     \If{$P_m > \tau$}
%     \State $k \gets \sum_{t=1}^n \mathbb{1}_{S_t < \:\rho}$
%     \State $\mathcal{U} \gets $ bottom $k$ token indices of $X_m$ w.r.t $S_t$
%     \State $\mathcal{V} \gets $ top $k$ token indices of $\tilde{X}_m$ w.r.t $S_t$
%     \Else
%     \State do not perform mix-up
%     \EndIf
%     \EndFor
    
    
%     \If{$p_m > \tau$}
%     \State $X^{(i)}, Y^{(i)} \gets X_s, Y_s$
%     \State $X^{(j)}, Y^{(j)} \gets \textrm{randomly sampled instance within batch}$
%     \State replace bottom $k$ tokens of $X^{(i)}$ with top $k$ tokens of $X^{(j)} $ w.r.t $\:\: s_t \:\: (t=1,2,\ldots,n)$
%     \State $\mathcal{U} \gets $ indices of unreplaced tokens of $X^{(i)}$
%     \State $\mathcal{V} \gets $ indices of borrowed tokens of $X^{(j)}$
%     \State $Y^{(i)} \gets \displaystyle \frac{\sum_{t=1}^n \mathbb{1}_{t \in \mathcal{U}} \cdot s_t^{(i)}}{\sum_{t=1}^n \mathbb{1}_{t \in \mathcal{U}} \cdot s_t^{(i)} +\sum_{t=1}^n \mathbb{1}_{t \in \mathcal{V}} \cdot s_t^{(j)}}\cdot Y^{(i)} + \frac{\sum_{t=1}^n \mathbb{1}_{t \in \mathcal{V}} \cdot s_t^{(j)}}{\sum_{t=1}^n \mathbb{1}_{t \in \mathcal{U}} \cdot s_t^{(i)} +\sum_{t=1}^n \mathbb{1}_{t \in \mathcal{V}} \cdot s_t^{(j)}} \cdot Y^{(j)}$
%     \State $X_s, Y_s \gets X^{(i)}, Y^{(i)}$
%     \Else
%     \State do not perform mix-up
%     \EndIf
%     \State \textbf{return} $X$, $Y$, $\textrm{CrossEntropyLoss}(\hat{y}, y)$
% \end{algorithmic}
% \end{algorithm}

==> Algorithms/htm_v2_full.tex <==

\begin{algorithm}[ht!]
\caption{Horizontal TokenMixup -- Full Version}
\label{alg:htm_v2_full}
\textbf{Input:} $X \in \rm I\!R^{b \times n \times d}$, $Y \in \rm I\!R^{b \times c}$, $\mathcal{T}$, $\tau$, $\rho$\\
\textbf{Output:} $Z \in \rm I\!R^{b \times n \times d}$, $Y, \hat{Y} \in \rm I\!R^{b \times c}$
\begin{algorithmic}[1]
    \State $A \gets \textrm{apply attention rollout for next }\ell$ layers
    % \State $A \gets \textrm{forward self attention with stop-gradient to retrieve attention map}$
    \State $S_t \gets \frac{1}{n}\sum_{i=1}^n  A_{i,t} \:\:\:\:\:\: \textrm{s.t.} \:\: t=1,2,\ldots,n$
    \State $\hat{Y} \gets \textrm{ScoreNet}(X)$
    \State $P \gets \textrm{CrossEntropy(Softmax}(\hat{Y}/\mathcal{T}), Y)$
    \State idx $\gets $ sample indices where $P > \tau$
    \State $b' \gets \textrm{number of items in idx}$
    \State $\tilde{X}, \tilde{Y}, \tilde{S} \gets X[\textrm{idx}], Y[\textrm{idx}], S[\textrm{idx}]$
    \State $C_{ij} \gets \sum_{t} \textrm{max}(\tilde{S}_t^{(j)} - {S}_t^{(i)},\: \rho) \:\:\:\:$ s.t. $i = 1, 2, \ldots, b$ and $j = 1, 2, \ldots, b'$
    \State $\sigma(m) \gets \textrm{HungarianMatching}(C_{ij})\:\:\:\:$ s.t. $m = 1, 2, \ldots, b'$  and $\sigma (m) \in \{1, 2, \ldots, b\}$
    \For{sample index $m = 1, 2, \ldots, b'$}
    \State $M_t \gets 0 \;\; \textrm{ if } S_t^{(\sigma(m))} - \tilde{S}_t^{(m)} > \rho \;\; \textrm{ else } 1 \:\:\:\:$ s.t. $t = 1, 2, \ldots, n$
    \State $\tilde{X}^{(m)} \gets M \odot \tilde{X}^{(m)} + (1-M) \odot X^{(\sigma(m))}$
    \State $\tilde{Y}^{(m)} \gets  \frac{\sum_t M_t \cdot \tilde{S}_t^{(m)}}{\sum_t M_t \cdot \tilde{S}_t^{(m)} + (1-M_t) \cdot S_t^{(\sigma(m))}} \tilde{Y}^{(m)} + \frac{\sum_t (1-M_t) \cdot S_t^{(\sigma(m))}}{\sum_t M_t \cdot \tilde{S}_t^{(m)} + (1-M_t) \cdot S_t^{(\sigma(m))}} Y^{(\sigma(m))}$
    \EndFor
    \State $X \gets \textrm{concatenate}(X[\neg \textrm{ idx}], \tilde{X}^{(m)}) \:\:\:\:$ s.t. $m = 1, 2, \ldots, b'$
    \State $Y \gets \textrm{concatenate}(Y[\neg \textrm{ idx}], \tilde{Y}^{(m)}) \:\:\:\:$ s.t. $m = 1, 2, \ldots, b'$
    \State $Z \gets \textrm{MultiHeadSelfAttention}(X)$
    \State \textbf{return } $Z$, $Y$, $\hat{Y}$
\end{algorithmic}
\end{algorithm}

==> Algorithms/hvtm.tex <==

\begin{minipage}{0.49\textwidth}
% \begin{adjustbox}{width=0.3\textwidth}
\begin{algorithm}[H]
\caption{Horizontal TokenMixup}
\footnotesize
\label{alg:htm}
\textbf{Input:} $X \in \rm I\!R^{b \times n \times d}$, $Y \in \rm I\!R^{b \times c}$, $\mathcal{T}$, $\tau$, $\rho$\\
\textbf{Output:} $Z \in \rm I\!R^{b \times n \times d}$, $Y, \hat{Y} \in \rm I\!R^{b \times c}$
\begin{algorithmic}[1]
    \State $A \gets \textrm{apply attention rollout for next }\ell$ layers
    % \State $A \gets \textrm{forward self attention with stop-gradient to retrieve attention map}$
    \State $S_t \gets \frac{1}{n}\sum_{i=1}^n  A_{i,t} \:\:\:\:\:\: \textrm{s.t.} \:\: t=1,2,\ldots,n$
    \State $\hat{Y} \gets \textrm{ScoreNet}(X)$
    \State $P \gets \textrm{CrossEntropy(Softmax}(\hat{Y}/\mathcal{T}), Y)$
    \State $\tilde{X}, \tilde{Y}, \tilde{S}_t \gets$ random permutation of $X, Y, S_t$
    \For{each sample index $m = 1, 2, \ldots, b$}
    \If{$P^{(m)} > \tau$}
    \State do not perform mixup
    \Else
    \State $k \gets \sum_{t=1}^n \mathbb{1}_{\{S_t^{(m)} < \:\rho\}}$
    \State $\mathcal{U} \gets $ bottom $k$ index of $X^{(m)}$  w.r.t \: $ S_t^{(m)}$
    \State $\mathcal{V} \gets $ top $k$ index of $\tilde{X}^{(m)}$ w.r.t \: $\tilde{S}_t^{(m)}$
    \State $X^{(m)}_{t \in \mathcal{U}} \gets \tilde{X}^{(m)}_{t \in \mathcal{V}} $  
    \State $Y^{(m)} \gets $ Relabel($Y^{(m)}, \tilde{Y}^{(m)}$)
    \EndIf
    \EndFor
    \State $Z \gets \textrm{MultiHeadSelfAttention}(X)$
    \State \textbf{return } $Z$, $Y$, $\hat{Y}$
\end{algorithmic}
\end{algorithm}
% \end{adjustbox}
\end{minipage}
\hfill
\begin{minipage}{0.49\textwidth}
\begin{algorithm}[H]
\caption{Vertical TokenMixup}
\footnotesize
\label{alg:vtm}
    \textbf{Input:} $X \in \rm I\!R^{b \times n \times d}$, $Y \in \rm I\!R^{b \times c}$, $L$, $\kappa$\\
    \textbf{Output:} $Z \in \rm I\!R^{b \times n \times d}$
\begin{algorithmic}[1]
    % \State $L \gets $ randomly select previous layer indices
    % \For{layer index $l \in L$}
    \For{layer index $l = 1, 2, \ldots, L-1$}
    \State $X^{(l)} \gets$ input tokens for layer $l$
    \State $A^{(l)} \gets \textrm{apply attention rollout for }\ell$ layers
    \State $S_t^{(l)} \gets \frac{1}{n}\sum_{i=1}^n  A_{i,t}^{(l)} \:\:\:\:\:\: \textrm{s.t.} \:\: t=1,2,\ldots,n$
    \State $X^{(l)}_\kappa \gets $ select top $\kappa$ tokens w.r.t \: $ S_t^{(l)}$
    \EndFor
    \State $X_{kv} \gets \textrm{concat}(X, X^{(l \in L)}_\kappa)$
    \State $X_{q} \gets X$
    \State $Z \gets \textrm{MultiHeadCrossAttention}(X_q, X_{kv})$
    \State \textbf{return } $Z$
\end{algorithmic}
\end{algorithm}
\end{minipage}

==> Algorithms/pseudocode_old.tex <==

\begin{algorithm}[h]
\caption{Query-Key Consistent Self-Attention -- Train Phase}
\label{alg:wamhsa_infer}
\begin{algorithmic}[1]
    \State \textbf{Input}  : $Q, K, V \in \rm I\!R^{N \times D}$, $\epsilon_1, \epsilon_2 \sim N(0,\sigma)$, sample number $n$
    \State \textbf{Output} : $Z \in \rm I\!R^{N\times D}$, consistency loss $\mathcal{L}_{con}$
    \State $\tilde{Q} \gets Q + \epsilon_1$
    \State $\tilde{K} \gets K + \epsilon_2$
    \State $idx \gets $ sample-idx$(n)$
    \If{random(0,1) < 0.5}
    \State $A \gets $ softmax$(\tilde{Q}\cdot K^\top / \tau)$
    \State $a_1 \gets A[idx]$
    \State $a_2 \gets $ softmax$(Q[idx]\cdot \tilde{K}^\top / \tau)$
    \Else
    \State $A \gets $ softmax$(Q\cdot \tilde{K}^\top / \tau)$
    \State $a_1 \gets A[idx]$
    \State $a_2 \gets $ softmax$(\tilde{Q}[idx]\cdot K^\top / \tau)$
    \EndIf
    \State $a_3 \gets $ softmax$(Q[idx]\cdot K^\top / \tau)$
    \State $Z \gets A \cdot V$
    \State $\mathcal{L}_{con} \gets $ MSE$(a1, a2) +$ MSE$(a2, a3) +$ MSE$(a1, a3)$
    \State \textbf{return} $Z, \mathcal{L}_{con}$
\end{algorithmic}
\end{algorithm}

% \begin{algorithm}[h]
% \caption{Wavelet Augmented Self Attention : Inference Phase}
% \label{alg:wamhsa_infer}
% \begin{algorithmic}[1]
%     \State \textbf{Input}  : $X \in \rm I\!R^{H \times W \times D}$, sample num $k$, radius $r$
%     \State \textbf{Output} : $Z \in \rm I\!R^{H \times W \times D}$
%     \State $P \gets $ topk(ScoreNet($X$), $k$)
%     \For{$p_i$ \textbf{in} $P$}
%     \State $X_i \gets $ crop($p_i$, $r$)
%     \State $A_i \gets X_i$
%     \State $B_i, C_i, D_i \gets $ Depthwise-Separable-Conv$(A)$
%     \State $X_i^{HR} \gets \mathcal{F}_{idwt}(A_i, B_i, C_i, D_i)$
%     \EndFor
%     \State $X^{HR} \gets$ concat$(X_i)$ \; s.t. $i = 1, ..., k$
%     \State $Z \gets $ WA-MHSA(query=$X$, key=$X \cup X^{HR}$, value=$X \cup X^{HR}$)
% \end{algorithmic}
% \end{algorithm}


% \begin{algorithm}[h]
% \caption{Wavelet Augmented Self Attention : Train Phase}
% \label{alg:wamhsa_train}
% \begin{algorithmic}[1]
%     \State \textbf{Input}  : $X \in \rm I\!R^{H \times W \times D}$, sample num $k$, radius $r$, loss coefficient $\beta$, $\xi$
%     \State \textbf{Output} : $Z \in \rm I\!R^{H \times W \times D}$, auxiliary loss $\mathcal{L}$
%     \State $\hat{A} \gets $ ScoreNet($X$)
%     \State $P \gets $ topk($\hat{A}, k$)
%     \For{$p_i$ \textbf{in} $P$}
%     \State $X_i \gets $ crop($p_i$, $r$)
%     \State $A_i \gets X_i$
%     \State $B_i, C_i, D_i \gets $ Depthwise-Separable-Conv$(A)$
%     \State $X_i^{HR} \gets \mathcal{F}_{idwt}(A_i, B_i, C_i, D_i)$
%     \EndFor
%     \State $X^{HR} \gets$ concat$(X_i)$ \; s.t. $i = 1, ..., k$
%     \State $Z, attn \gets $ WA-MHSA(query=$X$, key=$X \cup X^{HR}$, value=$X \cup X^{HR}$)
%     \State
%     \State $A \gets$ AvgPool($X$, stride=2)
%     \State $B, C, D \gets $ Depthwise-Separable-Conv$(A)$
%     \State $\hat{X} \gets \mathcal{F}_{idwt}(A,B,C,D)$
%     \State $\mathcal{L}_{recon} \gets$ MSEloss$(\hat{X}, X)$
%     \State $\mathcal{L}_{idwt} \gets $ MSEloss$(\mathcal{F}_{idwt}.weight, iDWT.weight)$
%     \State $\mathcal{L}_{score} \gets$ BCEloss$(\hat{A}, attn)$
%     \State $\mathcal{L} \gets \gamma \cdot \mathcal{L}_{recon} + \beta \cdot \mathcal{L}_{idwt} + \xi \cdot \mathcal{L}_{score}$
    
    
% \end{algorithmic}
% \end{algorithm}

==> Algorithms/vtm.tex <==
\begin{algorithm}[h!]
\caption{Vertical TokenMixup}
\label{alg:vtm}
\begin{algorithmic}[1]
    \State \textbf{Input:} $X \in \rm I\!R^{b \times n \times d}$, $Y \in \rm I\!R^{b \times c}$, $T$, $\kappa$
    \State \textbf{Output:} $Z \in \rm I\!R^{b \times n \times d}$
    \State $L \gets $ randomly select previous layer indices
    \For{layer index $l \in L$}
    \State $X^{(l)} \gets$ input tokens for layer $l$
    \State $A^{(l)} \gets \textrm{apply attention rollout for }\ell$ layers
    \State $S_t \gets \frac{1}{n}\sum_{i=1}^n  A_{t,i}^{(l)} \:\:\:\:\:\: \textrm{s.t.} \:\: t=1,2,\ldots,n$
    \State $X^{(l)}_\kappa \gets $ select top $\kappa$ tokens w.r.t \: $ S_t$
    \EndFor
    \State $X_{kv} \gets \textrm{concat}(X, X^{(l \in L)}_\kappa)$
    \State $X_{q} \gets X$
    \State $Z \gets \textrm{MultiHeadAttention}(X_q, X_{kv})$
    \State \textbf{return } $Z$
\end{algorithmic}
\end{algorithm}

==> Figures/tex/append_rollout.tex <==

\begin{figure}[h]
\begin{center}
\includegraphics[width=140mm]{Figures/img/append_rollout_v3_1.png}
\end{center}
\caption{\footnotesize \textbf{Additional qualitative examples}}
\label{fig:rollout_append}
\end{figure}

==> Figures/tex/dummy.tex <==
\begin{figure}[tp]
\begin{center}
\includegraphics[width=50mm]{Figures/img/dummy.png}
\end{center}
\caption{\textbf{Dummy}. }
\label{fig:dummy}
\end{figure}

==> Figures/tex/manifold.tex <==

\begin{figure}[h!]
\begin{center}
\includegraphics[width=\textwidth]{Figures/img/manifold.png}
\end{center}
\vspace{-3mm}
\caption{\footnotesize \textbf{Attention map comparison of HTM and Manifold Mixup.} 8 mixed pairs are sampled each for Horizontal TokenMixup and Manifold Mixup, to compare the attention map from the subsequent layer. Artifacts and smoothed attention heads (\textit{e.g.} head 1 \& 2) are observed for Manifold Mixup, which we believe is the reason Manifold Mixup did not perform well in our experiments.}
\label{fig:manifold}
\end{figure}

==> Figures/tex/scorenet.tex <==

\begin{figure}[h]
\begin{center}
\includegraphics[width=100mm]{Figures/img/scorenet.png}
\caption{\textbf{ScoreNet Architecture.} (left) ScoreNet for transformers that do not use \textit{cls} tokens. Each token is projected to a scalar value which serves as the attention weight for linear combination. Then, the linearly-combined token $X$ is used for classification. (right) If \textit{cls} token exists, we directly use the token for classification.}
\end{center}
\label{fig:scorenet}
\end{figure}
% \begin{minipage}{0.35\textwidth}
% \begin{figure}[H]
% \includegraphics[width=41mm]{Figures/img/scorenet.png}
% \end{center}
% \caption{\textbf{ScoreNet Architecture}. }
% \label{fig:scorenet}
% \end{figure}
% \end{minipage}
% \hfill
% \begin{minipage}{0.6\textwidth}
% \begin{figure}[H]
% \begin{center}
% \includegraphics[width=86mm]{Figures/img/htm.png}
% \end{center}
% \caption{\textbf{Horizontal TokenMixup}. }
% \label{fig:htm}
% \end{figure}
% \end{minipage}

==> Tables/adversarial.tex <==

\begin{table}[h]
    \centering
    \setlength{\tabcolsep}{3.5pt}
    \caption{\footnotesize\textbf{Robustness to Gaussian noise}}
    \vspace{-3mm}
        \begin{adjustbox}{width=\textwidth}
    \footnotesize
    \begin{tabular}[t]{l | c c c c c c}
    \toprule
    $\sigma$ & 0.0 & 0.1 & 0.2 & 0.3 & 0.4 & 0.5 \\
    \midrule
    baseline & 
    82.87 {\footnotesize(\textcolor{blue}{-0.00})} & 
    78.10 {\footnotesize(\textcolor{blue}{-4.77})} & 
    68.99 {\footnotesize(\textcolor{blue}{-13.88})} & 
    55.73 {\footnotesize(\textcolor{blue}{-27.14})}& 
    41.58 {\footnotesize(\textcolor{blue}{-41.29})}& 
    29.79 {\footnotesize(\textcolor{blue}{-53.08})} \\
    baseline + \textbf{Horizontal TM} & 
    \textbf{83.56} {\footnotesize(\textcolor{blue}{-0.00})} &
    \textbf{79.11} {\footnotesize(\textcolor{blue}{-4.45})}& 
    \textbf{71.60} {\footnotesize(\textcolor{blue}{-11.96})}&
    \textbf{60.71} {\footnotesize(\textcolor{blue}{-22.85})} & 
    \textbf{45.95} {\footnotesize(\textcolor{blue}{-37.61})}& 
    \textbf{32.34} {\footnotesize(\textcolor{blue}{-51.22})}\\
    baseline + \textbf{Vertical TM} & 
    83.54 {\footnotesize(\textcolor{blue}{-0.00})} &
    78.68 {\footnotesize(\textcolor{blue}{-4.86})}& 
    70.21 {\footnotesize(\textcolor{blue}{-13.33})}& 
    58.24 {\footnotesize(\textcolor{blue}{-25.30})}& 
    43.94 {\footnotesize(\textcolor{blue}{-39.60})}& 
    32.09 {\footnotesize(\textcolor{blue}{-51.45})} \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{tab:adversarial}
\end{table}


\begin{table}[h]
    \centering
    \setlength{\tabcolsep}{3.5pt}
    \caption{\footnotesize\textbf{Robustness to PGD attack}}
    \vspace{-3mm}
        \begin{adjustbox}{width=\textwidth}
    \footnotesize
    \begin{tabular}[t]{l | c c c c c}
    \toprule
    $\alpha$ & none & 0.001 & 0.003 & 0.010 & 0.030 \\
    \midrule
    baseline & 
    82.87 {\footnotesize(\textcolor{blue}{-0.00})} & 
    69.68 {\footnotesize(\textcolor{blue}{-13.19})} & 
    64.54 {\footnotesize(\textcolor{blue}{-18.33})} & 
    48.72 {\footnotesize(\textcolor{blue}{-34.15})}& 
    \textbf{30.05} {\footnotesize(\textcolor{blue}{-52.82})} \\
    baseline + \textbf{Horizontal TM} & 
    \textbf{83.56} {\footnotesize(\textcolor{blue}{-0.00})} &
    \textbf{70.94} {\footnotesize(\textcolor{blue}{-12.62})}& 
    \textbf{66.05} {\footnotesize(\textcolor{blue}{-17.51})}&
    \textbf{50.70} {\footnotesize(\textcolor{blue}{-32.86})} & 
    30.04 {\footnotesize(\textcolor{blue}{-53.52})}\\
    baseline + \textbf{Vertical TM} & 
    83.54 {\footnotesize(\textcolor{blue}{-0.00})} &
    70.47 {\footnotesize(\textcolor{blue}{-13.07})}& 
    65.13 {\footnotesize(\textcolor{blue}{-18.41})}& 
    49.40 {\footnotesize(\textcolor{blue}{-34.14})}& 
    29.59 {\footnotesize(\textcolor{blue}{-53.95})} \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{tab:pgd}
\end{table}


==> Tables/cifar.tex <==

\begin{table}[ht!]
    \centering
    \setlength{\tabcolsep}{3.5pt}
    \caption{\textbf{Experiment results on CIFAR.} \footnotesize Experiment results with TokenMixup on CCT are compared with state-of-the-art models that do not use pretrained models at initialization. Top-1 validation accuracy is reported for each model, and baseline models denoted with * reports retrained performance. Also, the number in the parenthesis indicates the number of epochs used for training.}
    \begin{adjustbox}{width=0.8\textwidth}
    \begin{tabular}{l@{\hskip 0.2in} |@{\hskip 0.1in} c c@{\hskip 0.1in} |@{\hskip 0.1in} c@{\hskip 0.1in} c@{\hskip 0.1in}}
        \toprule
        \textbf{Models} & \textbf{\# Params} & \textbf{MACs} & \textbf{CIFAR-10} & \textbf{CIFAR-100}  \\
        \midrule
        \midrule
        \multicolumn{5}{l}{\textit{Convolutional Network based}} \\ 
        \midrule
        ResNet18 & 11.18 M & 0.04 G & 90.27 & 63.41 \\
        % ResNet34 & 21.29 M & 0.08 G & 90.51 & 64.52 \\
        ResNet50 & 23.53 M & 0.08 G & 90.60 & 61.68 \\
        ResNet1001-v2~\cite{he2016identity} & 10.33 M & 1.55 G & 95.08 & 77.29 \\
        MobileNetV2/2.0~\cite{sandler2018mobilenetv2} & 8.72 M & 0.02 G & 91.02  & 67.44 \\
        WRN-28-10~\cite{zagoruyko2016wide} & 36.5 M & - & 96.00 & 80.75 \\
        WRN-40-4~\cite{zagoruyko2016wide} & 8.9 M & - & 95.47 & 78.82 \\
        ResNeXt-29-8×64d~\cite{xie2017aggregated} & 34.4 M & - & 96.35 & 82.23 \\
        ResNeXt-29-16×64d~\cite{xie2017aggregated} & 68.1 M & - & 96.42 & 82.69 \\
        \midrule
        \multicolumn{5}{l}{\textit{Transformer based}} \\ 
        \midrule
        % ViT-12/16 & 85.63 M & 0.43 G & 76.42 & 46.61 \\
        ViT-Lite-6/4~\cite{hassani2021escaping}  & 3.19 M & 0.21 G & 90.94 & 69.20 \\
        ViT-Lite-7/4~\cite{hassani2021escaping}  & 3.72 M & 0.24 G & 91.38 & 69.74 \\
        NesT-T~\cite{zhang2022nested} & 17.0 M & - & 96.04 & 78.69 \\
        NesT-B~\cite{zhang2022nested} & 68.0 M & - & 97.20 & 82.56 \\
        CVT-6/4~\cite{hassani2021escaping} & 3.19 M & 0.20 G & 92.58 & 72.25  \\
        CCT-7/3x1(1500)~\cite{hassani2021escaping}  & 3.76 M & 0.95 G & 97.48 & 82.72 \\
        CCT-7/3x1(1500) $^{*}$  & 3.78 M & 0.95 G &   & 83.07  \\
        CCT-7/3x1(1500) + \textbf{Horizontal TM (ours)} & 3.81 M  & 0.95 G & \textbf{97.65}  & \textbf{83.55}  \\
        CCT-7/3x1(1500) + \textbf{Vertical TM (ours)} & 3.78 M & 0.95 G & \textbf{97.84} & \textbf{83.42} \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{tab:cifar}
\end{table}


==> Tables/imagenet.tex <==

\begin{table}[ht!]
    \centering
    \setlength{\tabcolsep}{3.5pt}
    \caption{\textbf{Experiment results on ImageNet.} \footnotesize Experiment results with TokenMixup on ViT are compared. We report Top-1 and Top-5 validation accuracy on ImageNet-1K. For baseline, we used ViT-B/16 ($224\times224$) pretrained on ImageNet-21K. $^\dagger$ denotes the officially reported performance after fine-tuning on ImageNet-1K.}
    \begin{adjustbox}{width=0.8\textwidth}
    \begin{tabular}{l@{\hskip 0.3in} |@{\hskip 0.1in} c c@{\hskip 0.1in} |@{\hskip 0.2in} c@{\hskip 0.2in} c@{\hskip 0.2in}}
        \toprule
        \textbf{Models} & \textbf{\# Params} & \textbf{MACs} & \textbf{Top-1} & \textbf{Top-5}  \\
        \midrule
        \midrule
        \multicolumn{5}{l}{\textit{Convolutional Network based}} \\ 
        \midrule
        ResNet50~\cite{he2016deep} & 25.5 M & 4.3 G & 76.20 & - \\
        ResNet152~\cite{he2016deep} & 60.19 M & 11.58 G & 78.57 & - \\
        DenseNet-264~\cite{huang2017densely} & - & - & 79.20 & 94.71 \\
        WRN-50-2-bottleneck~\cite{zagoruyko2016wide} & 68.9 M & - & 78.10 & 93.97 \\
        ReGNetY-4G~\cite{radosavovic2020designing} & 21 M & 2.0 G & 80.0 & - \\
        ResNeXt-50-2×40d~\cite{xie2017aggregated} & - & - & 77.00 & - \\
        ResNeXt-101-64x4d~\cite{xie2017aggregated} & - & - & 79.60 & 94.70 \\
        \midrule
        \multicolumn{5}{l}{\textit{Transformer based}} \\ 
        \midrule
        ViT-B/16-224$^{\dagger}$ ~\cite{dosovitskiy2020image}  & 86.6 M & 16.9 G  & 81.2 & - \\
        ViT-B/16-224 + \textbf{Horizontal TM (ours)} & 87.3 M & 16.9 G &  \textbf{82.38} & \textbf{96.29} \\
        ViT-B/16-224 + \textbf{Vertical TM (ours)} & 86.6 M & 16.9 G & \textbf{82.31} & \textbf{96.30} \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{tab:imagenet}
\end{table}


==> Tables/otherarch.tex <==
\begin{table}[h]
\centering
\caption{\footnotesize \textbf{Experiments on other architectures.} TokenMixup methods are applied to other vision transformer architectures including ViT-Lite and PVTv2. * denotes the reproduced result.}
\vspace{-3mm}
\label{tab:otherarch}
    \begin{adjustbox}{width=0.49\textwidth}
    \footnotesize
    \begin{tabular}[t]{l | c}
        \toprule
       model & CIFAR-100 Accuracy \\
        \midrule
        ViT-Lite-7/4 (1500) $^*$~\cite{hassani2021escaping} & 79.44 \\
        ViT-Lite-7/4 (1500) + HTM & 80.53 \\
        ViT-Lite-7/4 (1500) + VTM & 80.44 \\
        ViT-Lite-7/4 (1500) + HTM + VTM & \textbf{80.65} \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{tab:vitlite}
    \hfill
    \begin{adjustbox}{width=0.49\textwidth}
    \footnotesize
    \begin{tabular}[t]{l | c c}
        \toprule
        model & ImageNet-1k Top1 & ImageNet-1k Top5 \\
        \midrule
        PVTv2-B0~\cite{wang2021pyramid} & 70.46 & 90.16 \\
        PVTv2-B0 + HTM & \textbf{71.20} & \textbf{90.43} \\
        PVTv2-B0 + VTM & - & - \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{tab:pvt}
\end{table}

==> Tables/random_sample.tex <==
\begin{table}[h]
\centering
\caption{\footnotesize \textbf{Comparison with random sample selection}}
\label{tab:random_token}
\begin{adjustbox}{width=0.4\textwidth}
\begin{tabular}{c|cc}
\hline
\rule{0pt}{1.0\normalbaselineskip}
Mixup type &  Accuracy &  Latency (ms)
\rule{0pt}{1.0\normalbaselineskip}\\
\hline
\rule{0pt}{1.0\normalbaselineskip}
Random & 82.12 & 85
\rule{0pt}{1.0\normalbaselineskip}\\
\rule{0pt}{1.0\normalbaselineskip}
HTM (Ours) & \textbf{83.56} & 89 
\rule{0pt}{1.0\normalbaselineskip}\\
\hline
\end{tabular}
\end{adjustbox}
\end{table}

==> Tables/random_token.tex <==
\begin{table}[h]
\centering
\caption{\footnotesize \textbf{Comparison with random token selection}}
\label{tab:random_baseline}
\begin{adjustbox}{width=0.4\textwidth}
\begin{tabular}{c|cc}
\hline
\rule{0pt}{1.0\normalbaselineskip}
Mixup type &  \textbf{Horizontal} &  \textbf{Vertical}
\rule{0pt}{1.0\normalbaselineskip}\\
\hline
\rule{0pt}{1.0\normalbaselineskip}
Random & 83.05 & 83.33 
\rule{0pt}{1.0\normalbaselineskip}\\
\rule{0pt}{1.0\normalbaselineskip}
Ours & \textbf{83.56} & \textbf{83.54} 
\rule{0pt}{1.0\normalbaselineskip}\\ 
\hline
\end{tabular}
\end{adjustbox}
\end{table}

==> Tables/saliency_random.tex <==
\begin{table}

\parbox{.59\linewidth}{
\centering
\caption{\footnotesize \textbf{Saliency detector comparison.} Our method achieves high accuracy while being twice as fast as the gradient method.}
\label{tab:saliency_map}
\begin{adjustbox}{width=0.6\textwidth}
\begin{tabular}{c|ccc}
\hline
\rule{0pt}{1.0\normalbaselineskip}
\cellcolor{gray!10}Saliency type & \cellcolor{gray!10}\textbf{Gradient-based} & \cellcolor{gray!10}\textbf{Attention Rollout} &\cellcolor{gray!10} \textbf{1-step Rollout} 
\rule{0pt}{1.0\normalbaselineskip}\\
\hline
\rule{0pt}{1.0\normalbaselineskip}
Avg. Latency (ms) & 346 (\textcolor{red}{+ 111.0\%}) & 211 (\textcolor{red}{+ 28.7\%}) & \cellcolor{yellow!25} 164 (+ 0.0\%) \rule{0pt}{1.0\normalbaselineskip}\\
\rule{0pt}{1.0\normalbaselineskip}
CIFAR-100 Acc. & 83.18 & 83.34 &\cellcolor{yellow!25} \textbf{83.55} 
\rule{0pt}{1.0\normalbaselineskip}\\
\hline
\end{tabular}
\end{adjustbox}
}
\hfill
\parbox{.39\linewidth}{
\centering
\caption{\footnotesize \textbf{Random baseline comparison.} Our methods outperform random baselines.}
\label{tab:random_baseline}
\begin{adjustbox}{width=0.31\textwidth}
\begin{tabular}{c|cc}
\hline
\rule{0pt}{1.0\normalbaselineskip}
\cellcolor{gray!10}Mixup type & \cellcolor{gray!10}\textbf{Horizontal} & \cellcolor{gray!10}\textbf{Vertical}
\rule{0pt}{1.0\normalbaselineskip}\\
\hline
\rule{0pt}{1.0\normalbaselineskip}
Random & 83.05 & 83.17 
\rule{0pt}{1.0\normalbaselineskip}\\
\rule{0pt}{1.0\normalbaselineskip}
Ours & \textbf{83.55} & \textbf{83.42} 
\rule{0pt}{1.0\normalbaselineskip}\\
\hline
\end{tabular}
\end{adjustbox}
}

\end{table}

==> Tables/scorenet.tex <==
\begin{table}[h]
\centering
\caption{\footnotesize \textbf{ScoreNet position analysis}}
\label{tab:scorenet}
\begin{adjustbox}{width=0.45\textwidth}
\begin{tabular}{c|cc}
\hline
\rule{0pt}{1.0\normalbaselineskip}
ScoreNet position &  Accuracy &  Latency$^*$ (ms)
\rule{0pt}{1.0\normalbaselineskip}\\
\hline
\rule{0pt}{1.0\normalbaselineskip}
final layer & 83.11 & 175
\rule{0pt}{1.0\normalbaselineskip}\\
\rule{0pt}{1.0\normalbaselineskip}
Ours & \textbf{83.56} & 119
\rule{0pt}{1.0\normalbaselineskip}\\
\hline
\end{tabular}
\end{adjustbox}
\end{table}

==> Tables/sensitivity_tbl.tex <==

\begin{table}[h]
    \centering
    \setlength{\tabcolsep}{3.5pt}
    \caption{ \footnotesize \textbf{Sample difficulty and saliency thresholds.} (left) CIFAR-100 performance with respect to sample difficulty threshold $\tau$ is reported. We also report the average number of samples HTM is applied. (middle) HTM performance with respect to saliency difference threshold $\rho$ is reported. We also report the average number of tokens mixed after convergence. (right) VTM performance by token sampling number per layer, $\kappa$, is reported.}
    \begin{adjustbox}{width=0.298\textwidth}
    \footnotesize
    \begin{tabular}[t]{c c c}
        \toprule
        $\tau$ & Accuracy & Avg. Count \\
        \midrule
         0.00 & 83.13 & 0 \\
        %  0.5 & 83.42 & 0 \\
         0.10 & 83.30 & 29 \\
         0.15 & 83.07 & 616 \\
         0.20 & \textbf{83.56}  & 2,142 \\
         0.25 & 83.30 & 5,471 \\
         0.30 & 82.91 & 11,072 \\
         \textrm{max} & 82.85 & 50,000 \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{tab:tau}
    \hfill
    \begin{adjustbox}{width=0.31\textwidth}
    \footnotesize
    \begin{tabular}[t]{c c c}
        \toprule
        $\rho$ & Accuracy & Avg. Count \\
        \midrule
         0.000 & 83.13 & 116.01 \\
         0.001 & 83.51 & 78.76 \\
         0.003 & 83.17 & 31.87 \\
         0.005 & \textbf{83.56} & 14.89 \\
         0.007 & 83.19 & 7.64 \\
        %  0.009 &  &  \\
         0.010 & 82.75 & 1.46 \\
         \textrm{max} & 82.90 & 0.0  \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{tab:rho}
    \hfill
    \begin{adjustbox}{width=0.164\textwidth}
    \footnotesize
    \begin{tabular}[t]{c c c c c c c c c}
        \toprule
        $\kappa$ & Accuracy \\
        \midrule
         0 & 82.87 \\
         5 & 83.16  \\
         10 & 83.01  \\
         30 & 83.09 \\
         50 & 83.28 \\
         80 & \textbf{83.54} \\
         100 & 83.46 \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{tab:kappa}
\end{table}

==> Tables/sharpness.tex <==
\begin{table}[h]
\centering
\caption{\footnotesize \textbf{Saliency map distribution sharpness comparison.}}
\label{tab:sharpness}
\begin{adjustbox}{width=0.45\textwidth}
\begin{tabular}{c|cc}
\toprule
 & Attention-based & Gradient-based \\
 \midrule
Total Variation (L1)  & 0.5454 &	1.3176 \\
Total Variation (L2) &	0.1441 &	0.3910 \\
Variance &	4.88E-6	& 1.95E-5\\
\hline
\end{tabular}
\end{adjustbox}
\end{table}

==> Tables/sup_mixup_compare.tex <==
\begin{table}[h]
\centering
\caption{\footnotesize \textbf{Comparison with other Mixup methods.}}
\label{tab:sup_mixup}
\begin{adjustbox}{width=0.7\textwidth}
\begin{tabular}{l|cc}
\toprule
model & CIFAR-100 Accuracy & Train GPU Time (hrs) \\
\midrule
CCT-7/3x1(1500)  & 82.87 &	24.5 \\
\midrule
CCT-7/3x1(1500) + Manifold Mixup~\cite{verma2019manifold} & 80.08 & - \\
CCT-7/3x1(1500) + Puzzle Mix~\cite{kim2020puzzle} & \textbf{83.61} & 68.5 \\
CCT-7/3x1(1500) + Co-Mixup~\cite{kim2021co} & 82.11 & 184.0 \\
CCT-7/3x1(1500) + Horizontal TM & 83.56 & \underline{25.5} \\
CCT-7/3x1(1500) + Vertical TM & 83.54 & \textbf{25.0}  \\
CCT-7/3x1(1500) + HTM + VTM & \underline{83.57} & 26.0  \\
\hline
\end{tabular}
\end{adjustbox}
\end{table}
